Some Asymptotic Results of Gaussian Random Fields with Varying Mean Functions and the Associated Processes

In this paper, we derive tail approximations of integrals of exponential functions of Gaussian random fields with varying mean functions and approximations of the associated point processes. This study is motivated naturally by multiple applications such as hypothesis testing for spatial models, study of the distribution of Bayesian marginal likelihood and Bayes factor, and financial applications.

==> frontmatter.tex <==
\RequirePackage[aos,amsthm,amsmath]{imsart}
\RequirePackage[OT1]{fontenc}
%\RequirePackage{hypernat,mymathbbol}

\usepackage{amsfonts,latexsym,amssymb,mymathbbol,bm}
\usepackage{graphics,graphicx}
\usepackage[colorlinks=true,linkcolor=black,citecolor=black,urlcolor=black]{hyperref}
\usepackage{amsmath}
\usepackage{graphicx}
\usepackage{color}%
\newcommand{\jc}[1]{{{\small \sc \color{blue}(#1)}}}

\startlocaldefs
\def\:{:\,}
\def\definedby{\stackrel{\Delta}{=}}

\def\pr{{'}}
\def\prpr{{''}}
\def\s{\sigma}
\def\sec{\setcounter{equation}{0}\setcounter{figure}{0}}
\newcommand{\symbolindex}[3]{\label{#1}\nomenclature{#2}{#3, \pageref{#1}}}
%\label{alpha}\nomenclature{$\alpha$}{Greek alpha, \pageref{alpha}}%
\newcommand{\blowup}[1]{B(#1)}
\newcommand{\blowupfn}[2]{{#1}^{#2}}
\def\codimens{{\rm Codim}}
\def\z{\zeta}
\def\wishart{\text{Wishart}}
\def\Prob{\P}
\def\vphi{\varphi}
\def\intsn{\int_{S^{N-1}}}
%\def\indic{{\mymathbb{1}}}
%\def\indic{{{1}}}
\def\ARF{{\it ARF}}
\def\RFG{{\it RFG}}
\def\iGRF{{\it GRF}}
\def\smallmorseindex{\mbox{\small Ind}}
\def\morseindex{\mbox{\rm Ind}}
\def\smallmorseindex{\mbox{\rm{\small Ind}}}
%\def\index{\mbox{\rm index}}
%\def\bb{\mathcal}
\def\boldPsi{{\bold \Psi}}
\def\EC{Euler characteristic\ }
\def\ECs{Euler characteristics\ }
\def\EPC{Euler-Poincar\'e characteristic}
\def\EP{Euler-Poincar\'e\ }
\def\lla{\left\langle}
\def\rra{\right\rangle}
\def\lb{\left\{}
\def\rb{\right\}}
\def\a{\alpha}
\def\cU{{\cal U}}
\def\cT{{\cal T}}
\def\Pl{{\cal P_l}}
\def\Plplus{{\cal P_{l+1}}}
%\def\bb{\mathbb}
\def\bb{\mathbb }
\def\half{\frac{1}{2}}
\def\smallhalf{\mbox{ $\frac{1}{2}$}}
\def\smallquarter{\mbox{$\frac{1}{4}$}}
\def\smallthreequarter{\mbox{$\frac{3}{4}$}}
\def\BC{Borell-TIS}
\def\cal{\mathcal}
\def\ep{\varepsilon}
\def\samples{\epsilon}
\def\rejection{D}
%\def\Hess{{\mbox{\rm Hess}}}
\def\det{{\mbox{\rm det}}}
\def\smalldet{\mbox{\small det}}
\def\prpr{\prime\prime}
% \setcounter{}{0}  \setcounter{}{0} \setcounter{}{0}
%   \setcounter{}{0} \setcounter{}{0} }
\def\VC{Vapnick-\v Cerv\-onen\-kis}
\def\GKF{Gaussian Kinematic Formula\ }
\def\LK{Lipschitz-Killing}
\def\LKC{Lipschitz-Killing curvature\ }
\def\LKCs{Lipschitz-Killing curvatures\ }
\def\ni{\noindent}
\def\cM{\cal M}
\def\dM{\partial \cM}
\def\SK{S^{K-1}}
\def\VK{\mbox{Vol}_{K-1}}
\def\P{{\bb P}}
\def\E{{\bb E}}
\def\Pp{{\bb P}}
\def\Ee{{\bb E}}
\def\I{{\rm Ind}}
\def\IN{I_N}
\def\N{{ N}}
\def\Z{{\bb Z}}
\def\ZN{{\bb Z}^N}
\def\e{{\varepsilon}}
\def\p{\varphi}
\def\real{{\bb{R}}}
%\def\real{{\Re}}
\def\complex{\mathbb{C}}
\def\sTX{\sup_{t\in T}f_t}
\def\varPsi{\Psi}
\def\RN{\mathbb{R}^N}
\def\RNprime{\mathbb{R}^{N'}}
\def\RK{\mathbb{R}^K}
\def\Rk{\mathbb{R}^k}
\def\Rd{\mathbb{R}^d}
\def\BN{\mathbb{B}^N}
\def\BorelN{\cal B^N}
\def\sphere{S}
\def\GRF{{\it The Geometry of Random Fields}}
\def\C{\mathbb{C}}
\def\definedas{\stackrel{\Delta}{=}}
\def\equalinlaw{\stackrel{\cal L}{=}}
\def\eqindist{\stackrel{\cal L}{=}}
\def\convinprob{\stackrel{{\P}}{\to}}
\def\convas{\stackrel{a.s. }{\to}}
\def\convinltwo{\stackrel{L_2}{ \to}}
\def\Sam{Samorodnitsky}
%\def\sheet{\stackrel{\circ}{W}\hspace*{-0.02truein}}
\def\sheet{W^\circ}
%\def\sheet{{\cal W}}
\def\sheett{\sheet_t}
\def\sas{$S\alpha S$ }
\def\SaS{$S\alpha S$ }
\def\sd{\cal S_d}
\def\stwod{\cal S_{2d}}
\def\stwodp{\cal S_{2d,p}}
\def\sprimed{\cal S'_d}
\def\sprimetwod{\cal S'_{2d}}
\def\sprimetwodp{\cal S'_{2d,p}}
\def\sheetst{\sheet_{st}}
\def\sheetuv{\sheet_{uv}}
\def\sheets{\sheet_{s}}
\def\sheetf{\sheet_{F}}
\def\sheetg{\sheet_{G}}
\def\Ito{It\^o\ }
\def\Itos{It\^o's\ }
\def\diam{\mbox{diam}}
\def\Min{{\cal M}}
\def\implies{\Rightarrow}
\def\ann{A^{(n)}_\eta}
\def\fad{F_{A^{(n)}(\p )}}
\def\VC{Vap\-nik-\v Cerv\-onen\-kis\ }
\def\done{\delta_1}
\def\dtwo{\delta_2}
\def\suptinT{\sup_{t \in T}}
\def\aone{a_1}
\def\atwo{a_2}
\def\bone{b_1}
\def\btwo{b_2}
\def\xx{\mbox{$\mathbf x$}}
\def\rr{\mbox{$\mathbf r$}}
\newcommand{\Y}{\mbox{$\mathbf Y$}}
\newcommand{\YY}{\mbox{$\mathbf Y$}}
\newcommand{\yy}{\mbox{$\mathbf y$}}
\newcommand{\zz}{\mbox{$\mathbf z$}}
\newcommand{\sqbinom}[2]{\begin{bmatrix}#1 \\ #2 \end{bmatrix}}
\newcommand{\ssqbinom}[2]{{\mbox{\scriptsize $\sqbinom{#1}{#2}$ }}}
\def\CA{\cal A}
\def\CC{\cal C}
\def\bX{X}
\def\bR{R}
\def\ba{a}
\def\bu{u}
%\def\tt{\widetilde t}
\def\tg{\widetilde g}
\def\tf{\widetilde f}
\def\hft{\widehat f^t}
\def\hW{\widehat W}
\def\tu{\tilde u}
\def\tD{\tilde D}
\def\tv{\tilde v}
\def\tx{\tilde x}
\def\cJ{{\cal J}}
\def\cO{{\cal O}}
\def\cH{{\cal H}}
\def\dotsb{\dots}
%\def\proof{\vskip0.12truein\noindent {\bf Proof.} }
%\def\qed{\hfill \mbox{\rule{3mm}{3mm}}\newline}
\def\KFF{kinematic fundamental formula}

\def\qed{\hfill $\Box$\newline}
\def\qedplusline{\hfill $\Box$\newline}


\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}

\newcommand{\dimamb}{{\dim}(\ambient)}

\newcommand{\eex}{\end{exercise}}
\newcommand{\bex}{\begin{exercise}}

\newcommand{\lab}{\label}
\newcommand{\mynumber}{\marginpar}
%\newcommand{\mynumber}{{ }}
\def\bk{\hspace*{-0.05truein}}
\def\KL{Karhunen-Lo\`eve}
%\newcommand{\argmin}{{\rm argmin}}
%\newcommand{\argmax}{{\rm argmax}}


%\renewcommand{\theequation}{\thesection.\arabic{figure}}
\renewcommand{\theequation}{\thesection.\arabic{equation}}
\renewcommand{\thefigure}{\thesection.\arabic{figure}}
%\renewcommand{\thefigure}{\thechapter.\thesection.\arabic{figure}}
%\renewcommand{\thetheorem}{\thechapter.\thesection.\arabic{theorem}}
\newcommand{\ssspace}{\vskip0.2truein}
\newcommand{\fq}{{\cal F}^{(q)}}
\newcommand{\fqe}{\cal F^{(q)}_\varepsilon}
%\newcommand{\parxpar}{\|f\|}
\newcommand{\parxpar}{\sup_{t\in T} f(t)}
\newcommand{\hg}{{\widehat g}}
\newcommand{\smc}{\scshape}
\newcommand{\ECdiff}[1]{{\rm Diff}_{f,#1}(u)}
\newcommand{\Rr}{\mathbb{R}}
\newcommand{\Nn}{\mathbb{N}}
\newcommand{\eexp}{{\rm e}}
\newcommand{\Hh}{\mathbb{H}}
\newcommand{\Hess}{\nabla^2}
\newcommand{\inv}{^{-1}}

\newcommand{\zpr}{Z^{\prime}}
\newcommand{\vari}{{\rm Var}}
\newcommand{\covari}{{\rm Cov}}
\newcommand{\dtr}{{\rm det}}
%\newcommand{\half}{\frac{1}{2}}
\newcommand{\myvec}{{\rm vec}}
\newcommand{\sign}{\text{\rm sgn}}
\newcommand{\Tt}{{\cal T}}
\newcommand{\Tr}{{\rm Tr}}
\newcommand{\grass}{\bigwedge^*}
\newcommand{\grasssq}{\bigwedge^{*,*}}
\newcommand{\grad}{\nabla}
%\newcommand{\qed}{$\Box$}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\mink}{{\cal M}}
\newcommand{\hauss}{{\cal H}}
\newcommand{\schwartz}{{\cal S}}
\newcommand{\lips}{{\cal L}}
\newcommand{\vol}{{\rm Vol}}
\newcommand{\translate}{{\rm T}}
\newcommand{\con}{{\rm Cone}}
\newcommand{\dimens}{{\dim}}
\newcommand{\deter}{{\rm det}}
\newcommand{\detr}{{\rm detr}}
\newcommand{\define}{\definedas}
\newcommand{\ambienttube}{\widehat{M}}
%\newcommand{\support}{{\cal S}}
%\newcommand{\argmax}[1]{\mathop{{\rm argmax}}_{#1}}
%\newcommand{\argmin}[1]{\mathop{{\rm argmin}}_{#1}}
\newcommand{\argmax}{\mathop{{\rm argmax}}}
\newcommand{\argmin}{\mathop{{\rm argmin}}}
\newcommand{\interior}[1]{{#1}^{\circ}}
%\newcommand{\interior}[1]{\overset{\circ}{#1}}
\newcommand{\closure}[1]{\overline{#1}}
\newcommand{\ambient}{\widetilde{M}}
\newcommand{\Curv}{{\rm Curv}}
\newcommand{\reducedtangent}{T^{\text{red}}}
\newcommand{\simp}{{\cal K}}
\newcommand{\support}{{\cal S}}
\newcommand{\Tube}{{\rm Tube}}
\def\newnotation#1{\label{#1}}
\def\overset{\stackrel}
\def\text{\mbox}
\def\tf{\widetilde f}
\def\th{\widetilde h}
\def\tg{\widetilde g}

\newcommand\Cov{\mathop{\rm Cov}}
\newcommand\Var{\mathop{\rm Var}}
\newcommand\Corr{\mathop{\rm Corr}}
\newcommand\tr{{\rm tr}}
\newcommand\diag{\mathop{\rm diag}}
\newcommand\spn{{\rm span}}
\newcommand{\geometrynotationdef}[2]{\vskip0.15truein \noindent
{\bf #1}\newnotation {#2}\newline}
\newcommand{\geometrydef}[1]{\vskip0.15truein \noindent
{\bf #1}\newline}
\newcommand{\projection}{\pi_{\sqrt{n},n,k}}
\newcommand{\projectioncomp}{{\rm id} - \projection}
\newcommand{\baseset}{M}
\newcommand{\basedomain}{D}
\newcommand{\hittingset}{\projection^{-1}\basedomain}
\newcommand{\intersection}{\baseset \cap y^{-1} \basedomain}
\newcommand{\warp}{\sigma}
\newcommand{\canS}[1]{S(\real^{#1})}
\newcommand{\canR}[1]{\real^{#1}}
\newcommand{\graff}{{\rm Graff}}
\newcommand{\grassman}{{\rm Gr}}
\newcommand{\comment}[1]{{\sc #1}}
\newcommand{\commentme}[1]{{\sc COMMENT ME LATER: #1}}
\newcommand{\trho}{{\widetilde \rho}}
\newcommand{\Span}{{\rm span}}
\newcommand{\nggstratum}[2]{M_{#1#2}}
\newcommand{\lmap}{{\cal T}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\theoremstyle{theorem}
%\newtheorem{defn}[lem]{Definition}
%\newtheorem*{note}{Note}
%\newtheorem{cla}[lem]{Claim}
\newtheorem{theorem}{Theorem}[section]
 \newtheorem{Theorem}{Theorem}[section]
 \newtheorem{lemma}[theorem]{Lemma}
 \newtheorem{corollary}[theorem]{Corollary}
 \newtheorem{Corollary}[theorem]{Corollary}
 \newtheorem{proposition}[theorem]{Proposition}
 \newtheorem{Proposition}[theorem]{Proposition}
 \newtheorem{definition}[theorem]{Definition}
 \newtheorem{Definition}[theorem]{Definition}
 \newtheorem{defi}[theorem]{Definition}
 \newtheorem{rem}[theorem]{Remark}
 \newtheorem{prop}[theorem]{Proposition}
 \newtheorem{cor}[theorem]{Corollary}
 \newtheorem{remark}[theorem]{Remark}
 \newtheorem{Remark}[theorem]{Remark}
 \newtheorem{Observation}[theorem]{Observation}
\newtheorem{example}[theorem]{Example}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{algorithm}[theorem]{Algorithm}
\newcommand{\beq}{\begin{eqnarray}}
\newcommand{\eeq}{\end{eqnarray}}
\newcommand{\beqq}{\begin{eqnarray*}}
\newcommand{\eeqq}{\end{eqnarray*}}

\DeclareMathOperator{\kernel}{ker}
\DeclareMathOperator{\rk}{rank}
\DeclareMathOperator{\vspan}{span}
\DeclareMathOperator{\Max}{Max}
\DeclareMathOperator{\ran}{Range}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\im}{Im}
\DeclareMathOperator{\re}{Re}
\DeclareMathOperator{\aut}{Aut}
\DeclareMathOperator{\res}{res}
\DeclareMathOperator{\Log}{Log}
\DeclareMathOperator{\Diff}{Diff}
\DeclareMathOperator{\Ext}{Ext}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\Wh}{Wh}
\DeclareMathOperator{\Cat}{Cat}
\DeclareMathOperator{\B}{B}
\DeclareMathOperator{\Int}{Int}
\DeclareMathOperator{\Hom}{Hom}
%\DeclareMathOperator{\vol}{Vol}
\DeclareMathOperator{\tube}{Tube}
\DeclareMathOperator{\chull}{chull}
%\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\length}{length}
%\DeclareMathOperator{\sign}{sign}
%\DeclareMathOperator{\C}{C}
%\DeclareMathOperator{\CV}{CV}
\DeclareMathOperator{\lf}{lf}
\def\lra{\Longrightarrow}
%\def\C{\mathbb{C}}
\def\CP{\mathbb{CP}}
\def\N{\mathbb{N}}
\def\Q{\mathbb{Q}}
\def\R{\mathbb{R}}
\def\Z{\mathbb{Z}}
\def\D{\mathcal{D}}
\def\V{\mathcal{V}}
\def\Hy{\mathbb{H}}
\def\T{\Theta}
\def\Ta{\mathcal{T}}
\def\St{\mathcal{S}}
\def\S{\Sigma}
\def\H{\mathcal{H}}
\def\N{\mathcal{N}}
\def\O{\Omega}
\def\G{\Gamma}
\def\L{\Lambda}
\def\a{\alpha}
\def\b{\beta}
\def\d{\delta}
\def\e{\varepsilon}
\def\g{\gamma}
\def\l{\lambda}
\def\r{\rho}
\def\s{\sigma}
\def\t{\tau}
\def\th{\theta}
\def\x{\xi}
\def\z{\zeta}
\def\o{\mathfrak{o}}
\def\nin{\noindent}
\def\bd{\partial}
\def\vp{\varphi}
\def\ldc{\lfloor d\chi \rfloor}
\def\udc{\lceil d\chi \rceil}
%\input{defs}
\newcommand{\given}{\;|\;}
%\newcommand{\E}{\mathbb{E}} %expectation
\newcommand{\PP}{\mathbb{P}}
\newcommand{\cov}{\mathrm{cov}}
\newcommand{\mean}[1] {\E\left\{{#1}\right\}}
\newcommand{\cmean}[2] {\E\left\{#1\given #2\right\}}
\newcommand{\prob}[1]{\mathbb{P}\left(#1\right)}
%\newcommand{\ind}{\boldsymbol{\mathbbm{1}}} % indicator function
%\newcommand{\indic}{\boldsymbol{\mathbbm{1}}} % indicator function
\newcommand{\ind}{{\mymathbb{1}}} % indicator function
\newcommand{\indic}{{\mymathbb{1}}} % indicator function
%\newcommand{\bX}{{\mathbf{X}}}
\newcommand{\Xne}{\bX_{n,\epsilon}}
\newcommand{\LL}{{\mathcal{L}}}
\newcommand{\MM}{{\mathcal{M}}}
\newcommand{\MMG}{{\mathcal{M}}^\gamma}
%-------- Parentheses
\newcommand{\size}[1]{\left|#1\right|}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\sbrk}[1]{\left[#1\right]}
\newcommand{\paren}[1]{\left(#1\right)}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\param}[1]{\left(#1\right)}
\newcommand{\abs}[1] {\left| {#1}\right|}
\newcommand{\floor}[1] {\left\lfloor{#1}\right\rfloor}
\newcommand{\ceil}[1] {\left\lceil{#1}\right\rceil}
\newcommand{\iprod}[1] {\left< {#1}\right>}
%\newcommand{\grad}{\triangledown}
\newcommand{\cP}{{\mathcal{P}}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cech}{\v{C}ech }
%\newcommand{\EC}{{Euler characteristic}}
\newcommand{\EI}{{Euler integral}}
\newcommand{\conv}{{\mathrm{conv}}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bt}{\mathbf{t}}
\def\w{\omega}
\newcommand{\comb}[2]{{{#1}\atopwithdelims[]{#2}}}
\newcommand{\hN}{\hat{N}}
\newcommand{\proofsmodea}[1]{{#1}}
\newcommand{\proofsmodeb}[1]{{aaa}}
\numberwithin{equation}{section}
\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\endlocaldefs

